Reproducible Science with LaTeX

This paper proposes a procedure to execute external source codes from a LaTeX document and include the calculation outputs in the resulting Portable Document Format (pdf) file automatically. It integrates programming tools into the LaTeX writing tool to facilitate the production of reproducible research. In our proposed approach to a LaTeX-based scientific notebook the user can easily invoke any programming language or a command-line program when compiling the LaTeX document, while using their favorite LaTeX editor in the writing process. The required LaTeX setup, a new Python package, and the defined preamble are discussed in detail, and working examples using R, Julia, and MatLab to reproduce existing research are provided to illustrate the proposed procedure. We also demonstrate how to include system setting information in a paper by invoking shell scripts when compiling the document.

==> tmp/initjulia.tex <==
 ┌ Warning: RCall.jl: Loading required package: igraph
│ 
│ Attaching package: ‘igraph’
│ 
│ The following objects are masked from ‘package:stats’:
│ 
│     decompose, spectrum
│ 
│ The following object is masked from ‘package:base’:
│ 
│     union
│ 
└ @ RCall ~/.julia/packages/RCall/Qzssx/src/io.jl:160



==> tmp/initprog.tex <==

Attaching package: ‘igraph’

The following objects are masked from ‘package:stats’:

    decompose, spectrum

The following object is masked from ‘package:base’:

    union



==> tmp/latexnb_inln3.tex <==
0.77


==> tmp/latexnb_inln7.tex <==
 Peter Hall, Raymond J Carroll, Jianqing Fan, Joseph G Ibrahim, T Tony Cai, David Dunson, Hua Liang, Jing Qin, Donglin Zeng, Hans-Georg Muller, Hongtu Zhu, Enno Mammen, Jian Huang, Runze Li, Song Xi Chen


==> tmp/latexnb_tmp5.tex <==
/home/ossifragus/Desktop/latexnb 
 initjulia.tex initprog.tex JiJin2016fig6.pdf JiJin2016fig6.tex latexnb_inln3.tex latexnb_inln7.tex latexnb_tmp5.tex latexnb_tmp8.tex LC-citations.pdf paperYear.tex propCitation.pdf sysinfo.tex table2.tex temp00.R 


==> tmp/latexnb_tmp8.tex <==
The input file matlabinterim doesn't exist


==> tmp/paperYear.tex <==
paperYear
2003 2004 2005 2006 2007 2008 2009 2010 2011 2012 
 296  320  328  354  350  370  409  355  325  141 


==> tmp/sysinfo.tex <==
Sat 03 Oct 2020 11:25:15 PM EDT

System Information
==================

Software versions
=================

R session information
=====================
R version 4.0.2 (2020-06-22)
Platform: x86_64-pc-linux-gnu (64-bit)
Running under: Ubuntu 20.04.1 LTS

Matrix products: default
BLAS:   /usr/lib/x86_64-linux-gnu/blas/libblas.so.3.9.0
LAPACK: /usr/lib/x86_64-linux-gnu/lapack/liblapack.so.3.9.0

locale:
 [1] LC_CTYPE=en_US.UTF-8       LC_NUMERIC=C              
 [3] LC_TIME=en_US.UTF-8        LC_COLLATE=en_US.UTF-8    
 [5] LC_MONETARY=en_US.UTF-8    LC_MESSAGES=en_US.UTF-8   
 [7] LC_PAPER=en_US.UTF-8       LC_NAME=C                 
 [9] LC_ADDRESS=C               LC_TELEPHONE=C            
[11] LC_MEASUREMENT=en_US.UTF-8 LC_IDENTIFICATION=C       

attached base packages:
[1] stats     graphics  grDevices utils     datasets  methods   base     

other attached packages:
[1] igraph_1.2.5  ineq_0.2-13   Matrix_1.2-18

loaded via a namespace (and not attached):
[1] compiler_4.0.2  magrittr_1.5    grid_4.0.2      pkgconfig_2.0.3
[5] lattice_0.20-41

Matlab version
==============
 /usr/local/MATLAB/R2020a

Julia version
=============
julia version 1.5.2

pdfTex version
==============
pdfTeX 3.14159265-2.6-1.40.20 (TeX Live 2019/Debian)
kpathsea version 6.3.1
Copyright 2019 Han The Thanh (pdfTeX) et al.
There is NO warranty.  Redistribution of this software is
covered by the terms of both the pdfTeX copyright and
the Lesser GNU General Public License.
For more information about these matters, see the file
named COPYING and the pdfTeX source.
Primary author of pdfTeX: Han The Thanh (pdfTeX) et al.
Compiled with libpng 1.6.37; using libpng 1.6.37
Compiled with zlib 1.2.11; using zlib 1.2.11
Compiled with xpdf version 4.01


==> tmp/table2.tex <==
\begin{table}

\caption{\label{tab:jj2016table2}Reproducing Table 2 from Ji and Jin, 2016}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{l|l|l|l|l}
\hline
\# of papers & \# of coauthors & \# of citers & Closeness & Betweenness\\
\hline
Peter Hall & Peter Hall & Jianqing Fan & Raymond J Carroll & Raymond J Carroll\\
\hline
Jianqing Fan & Raymond J Carroll & Hui Zou & Peter Hall & Peter Hall\\
\hline
Raymond J Carroll & Joseph G Ibrahim & Peter Hall & Jianqing Fan & Jianqing Fan\\
\hline
\end{tabular}}
\end{table}

